Unlocking datasets by calibrating populations of models to data density: a study in atrial electrophysiology

The understanding of complex physical or biological systems nearly always requires a characterisation of the variability that underpins these processes. In addition, the data used to calibrate such models may also often exhibit considerable variability. A recent approach to deal with these issues has been to calibrate populations of models (POMs), that is multiple copies of a single mathematical model but with different parameter values. To date this calibration has been limited to selecting models that produce outputs that fall within the ranges of the dataset, ignoring any trends that might be present in the data. We present here a novel and general methodology for calibrating POMs to the distributions of a set of measured values in a dataset. We demonstrate the benefits of our technique using a dataset from a cardiac atrial electrophysiology study based on the differences in atrial action potential readings between patients exhibiting sinus rhythm (SR) or chronic atrial fibrillation (cAF) and the Courtemanche--Ramirez--Nattel model for human atrial action potentials. Our approach accurately captures the variability inherent in the experimental population, and allows us to identify the differences underlying stratified data as well as the effects of drug block.

==> commands.tex <==
\newcommand{\pde}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdeb}[1]{\frac{\partial}{\partial #1}}
\newcommand{\pden}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}
\newcommand{\pdebn}[2]{\frac{\partial^{#2}}{\partial #1^{#2}}}
\newcommand{\de}[2]{\frac{d #1}{d #2}}
\newcommand{\deb}[1]{\frac{d}{d #1}}
\newcommand{\den}[3]{\frac{d^{#3} #1}{d #2^{#3}}}
\newcommand{\debn}[2]{\frac{d^{#2}}{d #1^{#2}}}
\newcommand{\refer}[1]{[\ref{#1}]}
\newcommand{\figref}[1] {Figure \ref{#1}}
\newcommand{\tabref}[1] {Table \ref{#1}}
\newcommand{\erfc}[1]{\mathrm{erfc}\left(#1\right)}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
